Stochastic Modeling of Hybrid Cache Systems

In recent years, there is an increasing demand of big memory systems so to perform large scale data analytics. Since DRAM memories are expensive, some researchers are suggesting to use other memory systems such as non-volatile memory (NVM) technology to build large-memory computing systems. However, whether the NVM technology can be a viable alternative (either economically and technically) to DRAM remains an open question. To answer this question, it is important to consider how to design a memory system from a "system perspective", that is, incorporating different performance characteristics and price ratios from hybrid memory devices. This paper presents an analytical model of a "hybrid page cache system" so to understand the diverse design space and performance impact of a hybrid cache system. We consider (1) various architectural choices, (2) design strategies, and (3) configuration of different memory devices. Using this model, we provide guidelines on how to design hybrid page cache to reach a good trade-off between high system throughput (in I/O per sec or IOPS) and fast cache reactivity which is defined by the time to fill the cache. We also show how one can configure the DRAM capacity and NVM capacity under a fixed budget. We pick PCM as an example for NVM and conduct numerical analysis. Our analysis indicates that incorporating PCM in a page cache system significantly improves the system performance, and it also shows larger benefit to allocate more PCM in page cache in some cases. Besides, for the common setting of performance-price ratio of PCM, "flat architecture" offers as a better choice, but "layered architecture" outperforms if PCM write performance can be significantly improved in the future.

==> background.tex <==
\section{Background and motivation} \label{sec:background}
\subsection{Page Cache}
Page cache is used to solve the high magnitude speed gap between memory and storage.
Traditional page cache use a large amount of DRAM size caching the recent-referenced file pages,
considering these data will be requested again in the near future, so that the following requests has a
large chance being served in memory without accessing the storage.
This is done transparently so that the applications will not notice any
difference to from where the data originate.

The demand of page cache is still increasing, especially
in enterprise server environment, typically a large amount of system
memory is used for caching contents in storage.
However, traditional DRAM-based page cache technology has difficult. DRAM scaling is in jeopardy
as charge storage and sensing mechanisms will become less reliable when scaled to thinner
manufacturing processes \cite{raoux2008phase}. Besides, it is shown that DRAM-based main memory spends a significant
portion of the total system cost and energy with the increasing size \cite{kgil2008improving}.
Therefore, a lot of work has been concentrating on studying new memory technologies that can be a candidate to DRAM.
%When the a file accessing request is coming, it will first check the page cache whether the page is already in memory.
%If the requested page is in page cache, then the request is served in memory copying request size of data to user space.
%Otherwise it will firstly trigger data copy from storage to memory, and then serve the request in cache.
%%which cost a additional delay in reading from storage compared to the first condition.
\subsection{Phase Change Memory}
Due to recent advances in non-volatile memory technologies such as PCM
(phase-change memory) or STT-MRAM (spin torque transfer magnetic RAM),
non-volatile memory is expected to be used as main memory of computer systems in the near future \cite{ISCA09}\cite{zhou2009durable}\cite{lee2010phase}\cite{lee2011characterizing}\cite{proctor2012non}.
However, as non-volatile memory will not completely replace DRAM due to capability-price ratio, it is considered
only as an add-on component to enhance performance. In this work, We motivate our work in the context of PCM,
but the problems faced are common to other memory technologies too.

%In terms of cost per gigabyte (GB), PCM capacity is more expensive than flash-based SSD capacity
%but cheaper than DRAM capacity. Meanwhile, PCM latencies are faster than flash-based
%SSD but slower than DRAM.

%Integrating PCM into the conventional system-level memory:
Whether PCM should be integrated into the conventional system-level page cache remains a question.
PCM is expected to be a scalable technology with feature size comparable to DRAM cells.
Given the scaling advantage of PCM technology, PCM can enable a larger capacity file cache,
which allows more data be served in memory. However, the drawback is that the access time for PCM memory is
lengthy due to the under-developing industrial technique,eg.,for 4KB read performance, in 2011 \cite{akel2011onyx} reported 38 $\mu s$
and in 2014 \cite{FAST14} reported 6.7 $\mu s$, though development has been made, it is orders of magnitudes slower than DRAM.
This reinforces the need to consider PCM from a system perspective incorporation with its price and capability characteristics.



Characterizing the performance of page cache is complex, cause the number of possible architectural choice,
page replacement/migration strategies among devices and the configuration of devices capacity is near infinite.
In this work£¬we use an analytical model to analysis the impact of these choice to page performance.


\begin{figure}[!t]
\centering
\subfigure[Data flow in $Arch.$ $Flat$]
{\includegraphics[height=1.7in,width=2.6in]{./fig/flat.pdf}}
\subfigure[Data flow in $Arch.$ $Layered$] {\includegraphics[height=1.7in,width=2.6in]{./fig/layer.pdf}}
\caption{data flow}
\label{fig:dataflow}
\end{figure}

==> limitation.tex <==
\section{Limitaions and discuss}\label{sec:limitation}

Our study into the applicability of PCM devices in memory
setting has provided several insights. However, we acknowledge that
our analysis do have some limitation:

First, in latency formulation,
we ignore some other factors that may affect access latency.
We do not attempt to model the caches prefetching behavior or the parallelism of request,
hence our latency model will large than real system. However the guidelines will not change.

Second, given the limitations in our model method,
a server workload that uses a large working set of
100-1000 of gigabytes is not effective. We scaled
our workloads and system cache size accordingly.


Third, in our analysis model, we concentrate on the read request as we assume that the
small fraction of write request will make little impact to the guidelines on cache design.
Further, we perform trace-based simulations to validate the insights obtained
using a trace is consist of both read and write request.
The observation is in line with the earlier guideline given by numerical analysis.


%In this study, we approach PCM as memory rather than storage, and
%our evaluation is focused on average performance improvement.

